Differentiable Stripe Patterns for Inverse Design of Structured Surfaces

Stripe patterns are ubiquitous in nature and everyday life. While the synthesis of these patterns has been thoroughly studied in the literature, their potential to control the mechanics of structured materials remains largely unexplored. In this work, we introduce Differentiable Stripe Patterns -- a computational approach for automated design of physical surfaces structured with stripe-shaped bi-material distributions. Our method builds on the work by Knoppel and colleagues for generating globally-continuous and equally-spaced stripe patterns. To unlock the full potential of this design space, we propose a gradient-based optimization tool to automatically compute stripe patterns that best approximate macromechanical performance goals. Specifically, we propose a computational model that combines solid shell finite elements with XFEM for accurate and fully-differentiable modeling of elastic bi-material surfaces. To resolve non-uniqueness problems in the original method, we furthermore propose a robust formulation that yields unique and differentiable stripe patterns. %Finally, we introduce design space regularizers to avoid numerical singularities and improve stripe neatness We combine these components with equilibrium state derivatives into an end-to-end differentiable pipeline that enables inverse design of mechanical stripe patterns. We demonstrate our method on a diverse set of examples that illustrate the potential of stripe patterns as a design space for structured materials. Our simulation results are experimentally validated on physical prototypes.

==> 99_heap.tex <==

The user also provides a design objective encoding desired mechanical performance such as a compliance map (see definition below), desired deformed shape under given loads, or macromechanical elasticity properties.

The vector field gives rise to stripe patterns on the surface, which we interpret as a bi-material distribution. In practice, we manufacture this distribution by printing one of the two materials as stiff reinforcements on top of a given material, e.g., a textile.

In order to predict the performance of such a reinforced design, we model the bi-material distribution using an extended finite element (XFEM) approach that accounts for discontinuous deformations across material interfaces. Using this simulation model, we can evaluate the performance of any input vector field. 

Given the input vector field, we want to find a continuous phase field such that Z indicates the gradient of the field at any point. Complex phase here automatically ensures global continuity of coordinate function even for closed surfaces and periodic boundary conditions.

   

Why is the eigenvector with the smallest eigenvalue meaningful?
We cannot get an exact match for non-integrable vector fields, so we are looking for a solution that minimizes the mismatch. Trivially, a smaller vector field magnitude will decrease this error - with zero being the minimum. Since this solution is not useful, we ask for the unit-norm field that minimizes the error. Asking for unit length displacement that minimizes error leads precisely to an eigenvector with minimum eigenvalue. To see this, consider the constrained optimization problem described through the Lagrangian
\begin{equation}
\label{eq:Lagrangian}
\mathcal{L} = \frac12\bv^t\bH\bv + \frac12 \lambda(||\bv||^2-1)\ 
\end{equation}
The first-order optimality conditions require that 
\begin{equation}
    \bH\bv + \lambda\bv = \mathbf{0} \ .
\end{equation}
While this condition is obviously satisfied for any eigenpair $(\bv_i,\lambda_i)$, only the eigenvector $\bv_\mathrm{min}$ for the smallest eigenvalue $\lambda_\mathrm{min}$ is a true minimizer of the energy in (\ref{eq:Lagrangian}).






\subsection{Questions}

- What are we losing compared to forward stripe patterns? How about non-orientable cases?
- Why use complex numbers?
We want a scalar function $\alpha$ that varies along the vector field with frequency $\nu$. If the function is real-valued, it isn't possible to guarantee global continuity (why??)
- How explain step from "want stripes orthogonal to vector field" to "compute angle-valued function whose gradient is as close as possible to omega"?
- Why is non-orientable important, and is it the source of all the s discontinuities? Are those directly related to the double cover?

- The angle/phase should change along the vector field $Z$ band stay constant orthogonal to it. So ideally, we would have a function $\alpha(u,v)$ such that $\nabla \alpha(u,v)=Z(u,v)$ everywhere in the domain. But this is not possible unless $Z$ is integrable, i.e., it derives from a potential.


- Stripe patterns has global continuity at its core. But that is, it seems, only important when looking at closed surfaces - without continuity requirements, easier options might be available? One reason for us to still insist on continuity is if we want to impose periodic boundary conditions - here, the periodicity constraint is equivalent to  (or stronger than)  seamlessness on a 3D surface. Besides that, we also want to be able to design reinforcements on arbitrary 3D surfaces - see our garments and balloon examples.

Method in brief.
Given vector field as input on triangle mesh, one vector per vertex, generate pattern with stripes running orthogonal to Z. Looking for an angle-valued function such that da = w. Only exist if integrable, so instead look for function that minimizes mismatch |da-w|.


\begin{enumerate}
    \item {\bf Projection}. project the vector field $\bZ$ onto the edges of each incident edge to obtain $\omega$
    \item {\bf Hessian}. build Laplace-like matrix with entries depending on $\omega$
    \item {\bf Eigenvector}. Find eigenvector $\bv$ of $\bA$ with smallest eigenvalue, $\bA\bv=\lambda\bv$
    \item {\bf Stripe Pattern}. Compute stripe function based on $\bv$ and $\omega$
\end{enumerate}



The processing applied to eigenvector is differentiable,  but the relation between A and input vector field is not differentiable - but only in case of singularities.

\paragraph{Questions to Answer}
- Impact of singularities? Do those pose problems for differentiation
- Why not use the frequency space formulation by Tricard et al.? They use a stochastic approach based on so called phasor noise. While not a problem for their forward design methodology, the inverse material design strategy that we pursue here requires derivative information on how a given pattern changes as a function of the design parameters. In this context, it is very much unclear how to differentiate through the sampling operations required in the approach by Tricard et al..
- What effect does the frequency have on the mechanical behavior? For example, for the same amount of reinforcement material and parallel lines, does the number of lines matter? For the same number of lines, is the amount of material simply changing the stiffness in the transverse direction?
- Is it easy to provide the input required for our method? Even if a user has a good idea of the distribution of rigid directions, are there global effects that are hard to predict using only local properties? We should be able to say 'yes' to this question, as otherwise we wouldn't even need inverse design.

\section{Singularities}
There are different types of singularities in the stripe pattern pipeline, some of which require special attention for differentiation.

\paragraph{Sinks and Sources}
The input vector field is generally not divergence free, which means that some triangles will have non-zero divergence. Such sinks and sources require special treatment in the parameterization.

\paragraph{Branching Points}
Branching points occur whenever...
This must be distinguished from branches in the resulting reinforcement patterns, i.e., locations where branches split or merge, which do not lead to problems.

\paragraph{Zeros}
When $\Psi=0$, the derivative $d arg \psi= <d\psi,i\psi>/|\psi|^2$ is no longer defined.

\paragraph{The Sign Discontinuity}
One step in computing the energy is transporting a vector along an incident edge to a neighbor vertex to measure the angle between them (or something like that). Depending on the sign of the dot product between these to vectors, different energy terms are used. This switch itself is not differentiable, and the resulting energy expression is only $C^0$-continuous.
We therefore replace the discrete jump with a continuous transition that we model with a sigmoid function,
\begin{equation}
    \tilde{E} = sigmoid(angle) \hat{E},  
\end{equation}
where $\tilde{E}$ and $\hat{E}$ denote smoothed and non-smooth energies, respectively.

What are parameters here, and how does the smoothing affect the outcome of the patterns?


==> Homogenization.tex <==
\section{Homogenization}
\label{sec:Homogenization}

We base our simulation model on the concept of multiscale mechanics. In such a model, the deformation of a microscale heterogeneous material is averaged into the deformation of a macroscale squared unit cell. This unit cell represents the smallest repeating substructure of a material, which allows to study its complex mechanical behavior by prescribing macroscale deformations, and condensing its response into simple macromechanical properties such as an averaged Young modulus $E_\mathrm{macro}$.

We use our XFEM model as the base for our micromechanical model, and prescribe macromechanical deformations through the use of periodic boundary conditions, where deformed nodal positions and enrichments at the boundaries of the unit cell follow $\deformed_i^+=\deformed_i^-+\bm{u}$ and $\enriched_i^+=\enriched_i^-$. The translation vector $\bm{u}$ is used to prescribe linear deformations on the unit cell. By removing the DoFs $\deformed^+$ and $\enriched^+$, the unconstrained DoFs can be retrieved from the remaining DoFs $\deformed_c$ and $\enriched_c$ as $\deformed=\stripeconstrain \deformed_c + \bm{U}$ and $\enriched=\stripeconstrain \enriched_c$, where $\stripeconstrain$ is the same matrix used to constrain the stripe phases, and $\bm{U}$ is $\bm{u}$ repeated in vector form for each $\deformed_i$.

Next, we find the static equilibrium of our micromechanical model, constrained by our macromechanical model by solving the minimization problem

\begin{equation}
    \argmin_{\deformed_c,\enriched_c}U(\deformed_c,\enriched_c,\undeformed,\levelset),
\end{equation}

which is solved using Newton by iteratively solving the system

\begin{align}
    \stripeconstrain^T \frac{\partial^2 U}{\partial (\deformed,\enriched)_i^2} \stripeconstrain \Delta(\deformed,\enriched)_i &= -\stripeconstrain^T \frac{\partial U}{\partial (\deformed,\enriched)_i} \\
    (\deformed,\enriched)_{i+1} &= (\deformed,\enriched)_{i} + \Delta(\deformed,\enriched)_i
\end{align}

until $\bm{f}=-\stripeconstrain^T \frac{\partial U}{\partial (\deformed,\enriched)_i}=0$.

We estimate the Young modulus of a deformation prescribed by $\bm{U}$ as 

\begin{equation}
    E_\mathrm{macro}(\deformed_c,\enriched_c,\undeformed,\levelset) = \frac{U(\deformed_c,\enriched_c,\undeformed,\levelset)}{A_\mathrm{macro}h}\frac{1}{d^2},
\end{equation}

where $d$ is the directional stretch encoded in $\bm{U}$ and $A_\mathrm{macro}$ is the area of the unit cell.



==> MethodJuan.tex <==
\section{Patterns}

We synthesize our stripe patterns following the method developed by Kn\"{o}ppel \etal. Given a per-vertex unit vector field $\vfield_i$, we first solve for per-vertex phases defined as complex numbers $\phases_i$ that minimize the energy $E$ defined as,

\begin{align}
E_{ij} &= \| \phases_i - e^{\omega \imi}\phases_j \|^2\text{, and} \\
E &= \sum_{ij} E_{ij},
\end{align}

where $E_{i,j}$ is the energy defined at the edge connecting the vertices $i$ and $j$, and $\omega$ is the rotation required to parallel-transport the phase from node $i$ to $j$. This rotation is chosen to increase the phase where $\bm{p}$ is parallel to the edge, and to remain constant where $\bm{p}$ is orthogonal to the edge. In mathematical terms, $\omega$ is defined as

\begin{equation}
    \omega=\frac{1}{2}l_{ij}f\left[ \mathrm{cos}(\vfield_i-\theta_{ij})+\mathrm{cos}(\vfield_j-\theta_{ji})\right],
\end{equation}

where $l_{ij}$ is the length of the edge, $f$ is the frequency of the stripe pattern and $\theta_{ij}$ and $\theta_{ji}$ are angular coordinates of the edge defined at the vertices $i$ and $j$ respectively, where $\theta=0$ corresponds to the vector $(1,0)$, and $\theta_{ij}=\pi+\theta_{ji}$.

$E$ can be expressed in matrix form as $\frac{1}{2}\phases^T \stripeenergy \phases$, where $\stripeenergy=\frac{\partial^2{E}}{\partial \phases^2}$. Additionally, as part of our homogenization system, we enforce periodic boundary conditions, requiring phases on the boundary to match, such that $\phases^+=\phases^-$. We address this problem, by removing DoFs at the boundary corresponding to $\phases^+$, and constraining them to be the same as $\phases^-$ through the matrix $\stripeconstrain$. Given constrained phases $\phasesc$, their unconstrained counterpart can be retrieved as $\phases = \stripeconstrain \phases^c$.

The energy defined above has many minimizers, including the trivial solution $\phases=0$. To avoid, we add a constraint asking for a non-zero norm for $\phases$, resulting in the constrained minimization problem

\begin{align}
    S=&\argmin_{\phases} \phasesc^T\stripeconstrain^T \stripeenergy \stripeconstrain \phasesc \\
    &\text{s.t. } \phasesc^T \stripeconstrain^T \stripemass \stripeconstrain \phasesc =1,
\end{align}

which is solved as a generalized eigenvalue problem $\stripeconstrain^T \stripeenergy \stripeconstrain \phasesc = \lambda \stripeconstrain^T \stripemass \stripeconstrain \phasesc$ using Spectra and choosing the smallest eigenvalue pair.

\section{Model}

We base our cloth and reinforcement material model on a standard anisotropic StVK energy density for thin shells, given by

\begin{equation}
    \psi=\frac{1}{2}\tilde{\strain}^T\tilde{\sigma},
\end{equation}

in Voigt notation, where $\strain=\frac{1}{2}(\defg^T\defg-\bm{I})$, $\tilde{\strain}=(\strain_{xx}, \strain_{yy}, 2\strain_{xy}^T$ is the Green-Lagrange quadratic strain tensor with $\defg$ as the deformation gradient and $\bm{I}$ as the identity matrix, and $\tilde{\sigma}=\tilde{\material}\tilde{\strain}$ establishes a linear relationship between stress and strain, where $\tilde{\material}$ is the material tensor in Voigt notation, expressed as a symmetric $3\times3$ matrix, with 6 independent values controlling the anisotropy of the material. We use two different material tensors, $\tilde{\material}_\mathrm{textile}$ an orthotropic material to model the material of the textile, and $\tilde{\material}_\mathrm{reinforcement}$ an isotropic material to model the material of the reinforcements.

We discretize our simulation model as a triangle mesh with deformed nodal positions $\deformed$, undeformed nodal positions $\undeformed$ and a levelset with DoFs at nodal positions $\levelset$, which represent the distance of the nodal position to the reinforcement interface. For elements not crossed by the interface (all nodal $\levelset_i$ are positive or negative for the element), we interpolate the deformed nodal positions using standard linear shape functions as

\begin{equation}
    \deformed_e=\sum_{e,i}{N_i(\undeformed_e)\deformed_{e,i}}.
\end{equation}

These elements exhibit constant strain throughout the element and its elastic energy is given by $U_e=\int_\Omega \psi(\deformed_i,\undeformed_i) = hA_0(\undeformed_{i})\psi(\deformed_i,\undeformed_i)$, where $A_0$ is the undeformed area of the element, and $h$ is its thickness.

To avoid remeshing of the simulation mesh and to allow the same mesh to simulate different interfaces, we interpolate elements crossed by the interface using XFEM enrichment functions. We choose the ridge enrichment function, which has been extensively used to model weak discontinuities such as the ones governing the reinforcements. The enrichment function is given by

\begin{equation}
    M=\sum_{e,i}|N_i\levelset_{e,i}|-\left|\sum_{e,i}N_i\levelset_{e,i}\right|,
\end{equation}

with the corresponding interpolation function for the nodal positions

\begin{equation}
    \deformed_e=\sum_{e,i}{N_i(\undeformed_e)\deformed_{e,i}}+M\sum_{e,i}{N_i(\undeformed_e)\enriched_{e,i}},
\end{equation}
    
where $\enriched$ are additional DoFs. For our problem, an element can only be crossed by at most one interface, avoiding the need for more complex solutions. 

The strain in the enriched elements varies throughout the element, with a kink located at the interface. To properly integrate over these elements, we subdivide them into three sub-elements, and integrate each one of them numerically following a 3-point Gaussian rule. The total energy of the system is then given by

\begin{equation}
    U(\deformed,\enriched,\undeformed,\levelset)=\sum_e U_e(\deformed_e,\enriched_e,\undeformed_e,\levelset_e).
\end{equation}

\paragraph{Levelset}

To obtain the levelset $\levelset$, which is a distance function from the phases $\phases$ of the stripe design, we evaluate the angle given by the phase $\alpha_i = \mathrm{arg}(\phases_i)$, and sample it using a smoothed triangle wave
    
\begin{equation}
    \phi_i=1-\frac{2\mathrm{arccos}[(1-a_1)\mathrm{sin}( \alpha_i)]}{\pi}-a_2,
\end{equation}
    
where $a_1$ is a smoothing term, and $a_2$ determines the ratio of reinforcement to textile by vertically translating the function, and therefore the location of the interface.

\section{Optimization}

We are interested in finding pattern in reinforcement designs that match a prescribed macromechanical profile. More specifically, we are interested in finding vector fields $\vfield$ for which the Young modulus of the unit cell $E_\mathrm{macro}$ matches a desired target $E_\mathrm{target}$. To this end, we prescribe a least-squares design objective 

\begin{equation}
    T=(E_\mathrm{macro}(\deformed_c,\enriched_c,\undeformed,\levelset)-E_\mathrm{target})^2
\end{equation}

that measures how far we are from the desired target. We minimize this objective by using sensitivity analysis. Differentiating the objective function gives the expression

\begin{equation}
    \frac{dT}{d\vfield} = \frac{\partial T}{\partial \vfield} + \frac{\partial (\deformed,\enriched)}{\partial \vfield}\frac{\partial T}{\partial (\deformed,\enriched)},
\end{equation}

where $\frac{\partial (\deformed,\enriched)}{\partial \vfield}$ is the sensitivity of the static equilibrium. However, neither the static equilibrium, nor the objective depend directly on the vector field. Using the chain rule, this derivative is expanded into the more general expression

\begin{equation}
    \frac{dT}{d\vfield} = \frac{\partial \phases}{\partial \vfield}^T \frac{\partial \levelset}{\partial \phases}^T \left[\frac{\partial T}{\partial \levelset} + \frac{\partial (\deformed,\enriched)}{\partial \levelset}\frac{\partial T}{\partial (\deformed,\enriched)}\right],
\end{equation}

where the partial derivatives with respect to the levelset $\levelset$ can be directly computed. In this expression, the partial derivative $\frac{\partial \phases}{\partial \vfield}$ must be treated carefully, as the phases $\phases$ are obtained through solving an eigenvalue problem, and the derivative must be obtained numerically. A simple solution would be to obtain this derivative through sensitivity analysis of the Lagrangian $L=\phases^T\stripeenergy\phases-\lambda (\phases^T \stripemass \phases-1)$. However, $\lambda$ has geometric multiplicity 2, and therefore infinite eigenvectors satisfying the conditions for the same eigenvalue. To solve this problem, we propose a regularized Lagrangian

\begin{equation}
    L_\mathrm{regularized} = (\phases-\phases_0)^2+(\lambda-\lambda_0)^2-\bm{\mu}^T(\stripeenergy-\lambda\stripemass)\phases
\end{equation}

to obtain a search direction that asks the new $\phases$ and $\lambda$ to be as close as possible to the last's iteration $\phases_0$ and $\lambda_0$ while still satisfying the eigenvalue condition $(\stripeenergy-\lambda\stripemass)\phases=0$, with $\bm{\mu}$ as Lagrange multipliers. The first order optimality condition for this Lagrangian with respect to $\phases$, $\lambda$ and $\bm{\mu}$ is expressed as

\begin{equation}
    \bm{H}_\mathrm{regularized}=
    \begin{pmatrix}
    \bm{I} & \stripemass\bm{\mu} & \lambda\stripemass-A \\
    (\stripemass\bm{\mu})^T & 1 & (\stripemass\bm{\phases})^T \\
    \lambda\stripemass-A & \stripemass\bm{\phases} & 0
    \end{pmatrix}
    =0.
\end{equation}

We obtain the partial derivative $\frac{\partial \phases}{\partial \vfield}$ using sensitivity analysis, exploiting the fact that

\begin{equation}
    \frac{d\bm{g}_\mathrm{regularized}}{d\vfield}=\frac{\partial \bm{g}_\mathrm{regularized}}{\partial \vfield} + \bm{H}_\mathrm{regularized}\frac{\partial \phases}{\partial \vfield} = 0,
\end{equation}

where $\bm{g}_\mathrm{regularized}=(0,0,-\frac{\partial(\stripeenergy)}{\partial \vfield})^T$ is the gradient of the regularized Lagrangian, assuming that $\bm{\mu}=0$ for the initial guess. Rearranging this system, we get that


\begin{equation}
   \frac{\partial \phases}{\partial \vfield} = -  \bm{H}_\mathrm{regularized}^{-1} \frac{\partial \bm{g}_\mathrm{regularized}}{\partial \vfield}.
\end{equation}

Then, to obtain $\phases_{i+1}$, we proceed to solve the eigenvalue problem for the new vector field $\vfield_{i+1}$. This process gives us two orthogonal vectors with the same eigenvalue $\phases^{\perp_1}_{i+1}$ and $\phases^{\perp_2}_{i+1}$. We obtain the new eigenvector $\phases_{i+1}=a_1\phases^{\perp_1}_{i+1}+a_2\phases^{\perp_2}_{i+1}$, by minimizing the expression

\begin{equation}
    R=\|a_1\phases^{\perp_1}_{i+1}+a_2\phases^{\perp_2}_{i+1} - \phases_{i}\|^2
\end{equation}

with respect to the coefficients $a_1$ and $a_2$.

Lastly, we obtain the sensitivity matrix of the static equilibrium using standard sensitivity analysis as

\begin{equation}
    \frac{\partial (\deformed,\enriched)}{\partial \levelset} = - \left[\stripeconstrain^T \frac{\partial^2 U}{\partial (\deformed,\enriched)_i^2} \stripeconstrain\right]^{-1} \stripeconstrain^T\frac{\partial\bm{f}}{\partial{\levelset}}
\end{equation}

The expressions are rearranged to solve the sensitivity analysis problem using the adjoint method.

We solve the gradient-based minimization problem using L-BFGS.

\section{Overview of method}

\begin{description}
\item{Simplified version of stripes without non-linear interpolation}
\item{Search direction using a regularized Lagrangian with the initial vector as reference}
\item{Solid shells for simulation allows us to incorporate bending with X-FEM}
\item{Regularize optimization by penalizing lambda}
\end{description}


==> Theory.tex <==








